Unsupervised Anomaly Detection via Nonlinear Manifold Learning

Anomalies are samples that significantly deviate from the rest of the data and their detection plays a major role in building machine learning models that can be reliably used in applications such as data-driven design and novelty detection. The majority of existing anomaly detection methods either are exclusively developed for (semi) supervised settings, or provide poor performance in unsupervised applications where there is no training data with labeled anomalous samples. To bridge this research gap, we introduce a robust, efficient, and interpretable methodology based on nonlinear manifold learning to detect anomalies in unsupervised settings. The essence of our approach is to learn a low-dimensional and interpretable latent representation (aka manifold) for all the data points such that normal samples are automatically clustered together and hence can be easily and robustly identified. We learn this low-dimensional manifold by designing a learning algorithm that leverages either a latent map Gaussian process (LMGP) or a deep autoencoder (AE). Our LMGP-based approach, in particular, provides a probabilistic perspective on the learning task and is ideal for high-dimensional applications with scarce data. We demonstrate the superior performance of our approach over existing technologies via multiple analytic examples and real-world datasets.

==> 01_Ref.tex <==
@article{oune2021latent,
  title={Latent map Gaussian processes for mixed variable metamodeling},
  author={Oune, Nicholas and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={387},
  pages={114128},
  year={2021},
  publisher={Elsevier}
}


@article{luong2021adaptive,
  title={Adaptive cost-aware Bayesian optimization},
  author={Luong, Phuc and Nguyen, Dang and Gupta, Sunil and Rana, Santu and Venkatesh, Svetha},
  journal={Knowledge-Based Systems},
  volume={232},
  pages={107481},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{zong2018deep,
  title={Deep autoencoding gaussian mixture model for unsupervised anomaly detection},
  author={Zong, Bo and Song, Qi and Min, Martin Renqiang and Cheng, Wei and Lumezanu, Cristian and Cho, Daeki and Chen, Haifeng},
  booktitle={International conference on learning representations},
  year={2018}
}

@article{braei2004anomaly,
  title={Anomaly detection in univariate time-series: A survey on the state-of-the-art. arXiv 2020},
  author={Braei, M and Wagner, S},
  journal={arXiv preprint arXiv:2004.00433}
}
@inproceedings{zhu2011revisit,
  title={Revisit dynamic arima based anomaly detection},
  author={Zhu, Bonnie and Sastry, Shankar},
  booktitle={2011 IEEE Third International Conference on Privacy, Security, Risk and Trust and 2011 IEEE Third International Conference on Social Computing},
  pages={1263--1268},
  year={2011},
  organization={IEEE}
}

@article{chandola2009anomaly,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{edgeworth1887xli,
  title={Xli. on discordant observations},
  author={Edgeworth, Francis Ysidro},
  journal={The london, edinburgh, and dublin philosophical magazine and journal of science},
  volume={23},
  number={143},
  pages={364--375},
  year={1887},
  publisher={Taylor \& Francis}
}
@MISC{Gpytorch,
howpublished={\url{https://gpytorch.ai/}}
}

@article{RN783,
   author = {Bostanabad, R. and Kearney, T. and Tao, S. Y. and Apley, D. W. and Chen, W.},
   title = {Leveraging the nugget parameter for efficient Gaussian process modeling},
   journal = {International Journal for Numerical Methods in Engineering},
   volume = {114},
   number = {5},
   pages = {501-516},
   ISSN = {0029-5981},
   DOI = {10.1002/nme.5751},
   url = {<Go to ISI>://WOS:000428998100002},
   year = {2018},
   type = {Journal Article}
}

@inproceedings{RN649,
   author = {Tao, Siyu and Shintani, Kohei and Bostanabad, Ramin and Chan, Yu-Chin and Yang, Guang and Meingast, Herb and Chen, Wei},
   title = {Enhanced Gaussian Process Metamodeling and Collaborative Optimization for Vehicle Suspension Design Optimization},
   booktitle = {ASME 2017 International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
   publisher = {American Society of Mechanical Engineers},
   volume = {2B},
   type = {Conference Proceedings}
}

@article{wang2019outlier,
  title={Outlier detection based on Gaussian process with application to industrial processes},
  author={Wang, Biao and Mao, Zhizhong},
  journal={Applied Soft Computing},
  volume={76},
  pages={505--516},
  year={2019},
  publisher={Elsevier}
}
@article{zhong2008classifying,
  title={Classifying EEG for brain computer interfaces using Gaussian processes},
  author={Zhong, Mingjun and Lotte, Fabien and Girolami, Mark and L{\'e}cuyer, Anatole},
  journal={Pattern Recognition Letters},
  volume={29},
  number={3},
  pages={354--359},
  year={2008},
  publisher={Elsevier}
}
@article{braei2020anomaly,
  title={Anomaly detection in univariate time-series: A survey on the state-of-the-art},
  author={Braei, Mohammad and Wagner, Sebastian},
  journal={arXiv preprint arXiv:2004.00433},
  year={2020}
}

@article{rajabzadeh2016dynamic,
  title={A dynamic modeling approach for anomaly detection using stochastic differential equations},
  author={Rajabzadeh, Yalda and Rezaie, Amir Hossein and Amindavar, Hamidreza},
  journal={Digital Signal Processing},
  volume={54},
  pages={1--11},
  year={2016},
  publisher={Elsevier}
}

@article{yu2019unsupervised,
  title={Unsupervised online anomaly detection with parameter adaptation for KPI abrupt changes},
  author={Yu, Guang and Cai, Zhiping and Wang, Siqi and Chen, Haiwen and Liu, Fang and Liu, Anfeng},
  journal={IEEE Transactions on Network and Service Management},
  volume={17},
  number={3},
  pages={1294--1308},
  year={2019},
  publisher={IEEE}
}

@article{zhang2015low,
  title={A low-rank and sparse matrix decomposition-based Mahalanobis distance method for hyperspectral anomaly detection},
  author={Zhang, Yuxiang and Du, Bo and Zhang, Liangpei and Wang, Shugen},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={54},
  number={3},
  pages={1376--1389},
  year={2015},
  publisher={IEEE}
}

@inproceedings{sarafijanovic2019fast,
  title={Fast distance-based anomaly detection in images using an inception-like autoencoder},
  author={Sarafijanovic-Djukic, Natasa and Davis, Jesse},
  booktitle={International Conference on Discovery Science},
  pages={493--508},
  year={2019},
  organization={Springer}
}

@article{magyar2022spatial,
  title={Spatial outlier detection on discrete GNSS velocity fields using robust Mahalanobis-distance-based unsupervised classification},
  author={Magyar, B{\'a}lint and Kenyeres, Ambrus and T{\'o}th, S{\'a}ndor and Hajdu, Istv{\'a}n and Horv{\'a}th, Roland},
  journal={GPS Solutions},
  volume={26},
  number={4},
  pages={145},
  year={2022},
  publisher={Springer}
}

@article{hariri2019extended,
  title={Extended isolation forest},
  author={Hariri, Sahand and Kind, Matias Carrasco and Brunner, Robert J},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={33},
  number={4},
  pages={1479--1489},
  year={2019},
  publisher={IEEE}
}

@inproceedings{breunig2000lof,
  title={LOF: identifying density-based local outliers},
  author={Breunig, Markus M and Kriegel, Hans-Peter and Ng, Raymond T and Sander, J{\"o}rg},
  booktitle={Proceedings of the 2000 ACM SIGMOD international conference on Management of data},
  pages={93--104},
  year={2000}
}

@inproceedings{syarif2012unsupervised,
  title={Unsupervised clustering approach for network anomaly detection},
  author={Syarif, Iwan and Prugel-Bennett, Adam and Wills, Gary},
  booktitle={International conference on networked digital technologies},
  pages={135--145},
  year={2012},
  organization={Springer}
}

@inproceedings{gao2012unsupervised,
  title={An unsupervised anomaly detection approach for spacecraft based on normal behavior clustering},
  author={Gao, Yu and Yang, Tianshe and Xu, Minqiang and Xing, Nan},
  booktitle={2012 Fifth International Conference on Intelligent Computation Technology and Automation},
  pages={478--481},
  year={2012},
  organization={IEEE}
}
@article{pu2020hybrid,
  title={A hybrid unsupervised clustering-based anomaly detection method},
  author={Pu, Guo and Wang, Lijuan and Shen, Jun and Dong, Fang},
  journal={Tsinghua Science and Technology},
  volume={26},
  number={2},
  pages={146--153},
  year={2020},
  publisher={TUP}
}

@article{baur2021autoencoders,
  title={Autoencoders for unsupervised anomaly segmentation in brain MR images: a comparative study},
  author={Baur, Christoph and Denner, Stefan and Wiestler, Benedikt and Navab, Nassir and Albarqouni, Shadi},
  journal={Medical Image Analysis},
  volume={69},
  pages={101952},
  year={2021},
  publisher={Elsevier}
}

@article{fernando2021deep,
  title={Deep learning for medical anomaly detection--a survey},
  author={Fernando, Tharindu and Gammulle, Harshala and Denman, Simon and Sridharan, Sridha and Fookes, Clinton},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={7},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{tao2022deep,
  title={Deep learning for unsupervised anomaly localization in industrial images: A survey},
  author={Tao, Xian and Gong, Xinyi and Zhang, Xin and Yan, Shaohua and Adak, Chandranath},
  journal={IEEE Transactions on Instrumentation and Measurement},
  year={2022},
  publisher={IEEE}
}

@inproceedings{lee2020unsupervised,
  title={Unsupervised anomaly detection of the gas turbine operation via convolutional auto-encoder},
  author={Lee, Geunbae and Jung, Myungkyo and Song, Myoungwoo and Choo, Jaegul},
  booktitle={2020 IEEE International Conference on Prognostics and Health Management (ICPHM)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{hu2022video,
  title={Video anomaly detection based on 3D convolutional auto-encoder},
  author={Hu, Xing and Lian, Jing and Zhang, Dawei and Gao, Xiumin and Jiang, Linhua and Chen, Wenmin},
  journal={Signal, Image and Video Processing},
  volume={16},
  number={7},
  pages={1885--1893},
  year={2022},
  publisher={Springer}
}

@inproceedings{aytekin2018clustering,
  title={Clustering and unsupervised anomaly detection with l 2 normalized deep auto-encoder representations},
  author={Aytekin, Caglar and Ni, Xingyang and Cricri, Francesco and Aksu, Emre},
  booktitle={2018 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@inproceedings{latecki2007outlier,
  title={Outlier detection with kernel density functions},
  author={Latecki, Longin Jan and Lazarevic, Aleksandar and Pokrajac, Dragoljub},
  booktitle={MLDM},
  volume={7},
  pages={61--75},
  year={2007}
}

@article{glyn2022anomaly,
  title={Anomaly detection in streaming data with gaussian process based stochastic differential equations},
  author={Glyn-Davies, Alex and Girolami, Mark},
  journal={Pattern Recognition Letters},
  volume={153},
  pages={254--260},
  year={2022},
  publisher={Elsevier}
}

@article{glyn2022anomaly,
  title={Anomaly detection in streaming data with gaussian process based stochastic differential equations},
  author={Glyn-Davies, Alex and Girolami, Mark},
  journal={Pattern Recognition Letters},
  volume={153},
  pages={254--260},
  year={2022},
  publisher={Elsevier}
}

@article{hartigan1979algorithm,
  title={Algorithm AS 136: A k-means clustering algorithm},
  author={Hartigan, John A and Wong, Manchek A},
  journal={Journal of the royal statistical society. series c (applied statistics)},
  volume={28},
  number={1},
  pages={100--108},
  year={1979},
  publisher={JSTOR}
}

@article{hartigan1979algorithm,
  title={Algorithm AS 136: A k-means clustering algorithm},
  author={Hartigan, John A and Wong, Manchek A},
  journal={Journal of the royal statistical society. series c (applied statistics)},
  volume={28},
  number={1},
  pages={100--108},
  year={1979},
  publisher={JSTOR}
}
@inproceedings{pelleg1999accelerating,
  title={Accelerating exact k-means algorithms with geometric reasoning},
  author={Pelleg, Dan and Moore, Andrew},
  booktitle={Proceedings of the fifth ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={277--281},
  year={1999}
}

@inproceedings{wang2011improved,
  title={An improved K-Means clustering algorithm},
  author={Wang, Juntao and Su, Xiaolong},
  booktitle={2011 IEEE 3rd international conference on communication software and networks},
  pages={44--46},
  year={2011},
  organization={IEEE}
}
@inproceedings{nayini2017novel,
  title={A novel threshold-based clustering method to solve K-means weaknesses},
  author={Nayini, S Ehsan Yasrebi and Geravand, Somayeh and Maroosi, Ali},
  booktitle={2017 International Conference on Energy, Communication, Data Analytics and Soft Computing (ICECDS)},
  pages={47--52},
  year={2017},
  organization={IEEE}
}

@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}
@article{song2021spectral,
  title={Spectral--spatial anomaly detection of hyperspectral data based on improved isolation forest},
  author={Song, Xiangyu and Aryal, Sunil and Ting, Kai Ming and Liu, Zhen and He, Bin},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--16},
  year={2021},
  publisher={IEEE}
}

@article{karczmarek2021fuzzy,
  title={Fuzzy c-means-based isolation forest},
  author={Karczmarek, Pawe{\l} and Kiersztyn, Adam and Pedrycz, Witold and Czerwi{\'n}ski, Dariusz},
  journal={Applied Soft Computing},
  volume={106},
  pages={107354},
  year={2021},
  publisher={Elsevier}
}

@article{lv2021latent,
  title={Latent Gaussian process for anomaly detection in categorical data},
  author={Lv, Fengmao and Liang, Tao and Zhao, Jiayi and Zhuo, Zhongliu and Wu, Jinzhao and Yang, Guowu},
  journal={Knowledge-Based Systems},
  volume={220},
  pages={106896},
  year={2021},
  publisher={Elsevier}
}

@article{wang2019outlier,
  title={Outlier detection based on Gaussian process with application to industrial processes},
  author={Wang, Biao and Mao, Zhizhong},
  journal={Applied Soft Computing},
  volume={76},
  pages={505--516},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{amer2013enhancing,
  title={Enhancing one-class support vector machines for unsupervised anomaly detection},
  author={Amer, Mennatallah and Goldstein, Markus and Abdennadher, Slim},
  booktitle={Proceedings of the ACM SIGKDD workshop on outlier detection and description},
  pages={8--15},
  year={2013}
}

@article{pang2021deep,
  title={Deep learning for anomaly detection: A review},
  author={Pang, Guansong and Shen, Chunhua and Cao, Longbing and Hengel, Anton Van Den},
  journal={ACM computing surveys (CSUR)},
  volume={54},
  number={2},
  pages={1--38},
  year={2021},
  publisher={ACM New York, NY, USA}
}
@article{chalapathy2019deep,
  title={Deep learning for anomaly detection: A survey},
  author={Chalapathy, Raghavendra and Chawla, Sanjay},
  journal={arXiv preprint arXiv:1901.03407},
  year={2019}
}
@inproceedings{aytekin2018clustering,
  title={Clustering and unsupervised anomaly detection with l 2 normalized deep auto-encoder representations},
  author={Aytekin, Caglar and Ni, Xingyang and Cricri, Francesco and Aksu, Emre},
  booktitle={2018 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}
@article{zhang2022deep,
  title={Deep dual support vector data description for anomaly detection on attributed networks},
  author={Zhang, Fengbin and Fan, Haoyi and Wang, Ruidong and Li, Zuoyong and Liang, Tiancai},
  journal={International Journal of Intelligent Systems},
  volume={37},
  number={2},
  pages={1509--1528},
  year={2022},
  publisher={Wiley Online Library}
}

@inproceedings{ghafoori2020deep,
  title={Deep multi-sphere support vector data description},
  author={Ghafoori, Zahra and Leckie, Christopher},
  booktitle={Proceedings of the 2020 SIAM International Conference on Data Mining},
  pages={109--117},
  year={2020},
  organization={SIAM}
}

@book{lumley2010fundamentals,
  title={Fundamentals of aluminium metallurgy: production, processing and applications},
  author={Lumley, Roger},
  year={2010},
  publisher={Elsevier}
}

@article{kopper2020model,
  title={Model selection and evaluation for machine learning: deep learning in materials processing},
  author={Kopper, Adam and Karkare, Rasika and Paffenroth, Randy C and Apelian, Diran},
  journal={Integrating Materials and Manufacturing Innovation},
  volume={9},
  pages={287--300},
  year={2020},
  publisher={Springer}
}

@article{fan2020robust,
  title={Robust deep auto-encoding Gaussian process regression for unsupervised anomaly detection},
  author={Fan, Jinan and Zhang, Qianru and Zhu, Jialei and Zhang, Meng and Yang, Zhou and Cao, Hanxiang},
  journal={Neurocomputing},
  volume={376},
  pages={180--190},
  year={2020},
  publisher={Elsevier}
}

@article{chandola2009anomaly,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{garmaroodi2020detection,
  title={Detection of anomalies in industrial iot systems by data mining: Study of christ osmotron water purification system},
  author={Garmaroodi, Mohammad Sadegh Sadeghi and Farivar, Faezeh and Haghighi, Mohammad Sayad and Shoorehdeli, Mahdi Aliyari and Jolfaei, Alireza},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={13},
  pages={10280--10287},
  year={2020},
  publisher={IEEE}
}

@article{skomedal2020much,
  title={How much power is lost in a hot-spot? A case study quantifying the effect of thermal anomalies in two utility scale PV power plants},
  author={Skomedal, {\AA}smund F and Aarseth, Bj{\o}rn L and Haug, Halvard and Selj, Josefine and Marstein, Erik S},
  journal={Solar Energy},
  volume={211},
  pages={1255--1262},
  year={2020},
  publisher={Elsevier}
}

@book{mehrotra2017anomaly,
  title={Anomaly detection principles and algorithms},
  author={Mehrotra, Kishan G and Mohan, Chilukuri K and Huang, HuaMing},
  volume={1},
  year={2017},
  publisher={Springer}
}

@article{noto2012frac,
  title={FRaC: a feature-modeling approach for semi-supervised and unsupervised anomaly detection},
  author={Noto, Keith and Brodley, Carla and Slonim, Donna},
  journal={Data mining and knowledge discovery},
  volume={25},
  pages={109--133},
  year={2012},
  publisher={Springer}
}

@article{ruff2019deep,
  title={Deep semi-supervised anomaly detection},
  author={Ruff, Lukas and Vandermeulen, Robert A and G{\"o}rnitz, Nico and Binder, Alexander and M{\"u}ller, Emmanuel and M{\"u}ller, Klaus-Robert and Kloft, Marius},
  journal={arXiv preprint arXiv:1906.02694},
  year={2019}
}

@article{gornitz2013toward,
  title={Toward supervised anomaly detection},
  author={G{\"o}rnitz, Nico and Kloft, Marius and Rieck, Konrad and Brefeld, Ulf},
  journal={Journal of Artificial Intelligence Research},
  volume={46},
  pages={235--262},
  year={2013}
}

@article{villa2021semi,
  title={Semi-supervised anomaly detection algorithms: A comparative summary and future research directions},
  author={Villa-P{\'e}rez, Miryam Elizabeth and Alvarez-Carmona, Miguel A and Loyola-Gonzalez, Octavio and Medina-P{\'e}rez, Miguel Angel and Velazco-Rossell, Juan Carlos and Choo, Kim-Kwang Raymond},
  journal={Knowledge-Based Systems},
  volume={218},
  pages={106878},
  year={2021},
  publisher={Elsevier}
}
@article{xia2022gan,
  title={GAN-based anomaly detection: a review},
  author={Xia, Xuan and Pan, Xizhou and Li, Nan and He, Xing and Ma, Lin and Zhang, Xiaoguang and Ding, Ning},
  journal={Neurocomputing},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{pang2021toward,
  title={Toward deep supervised anomaly detection: Reinforcement learning from partially labeled anomaly data},
  author={Pang, Guansong and van den Hengel, Anton and Shen, Chunhua and Cao, Longbing},
  booktitle={Proceedings of the 27th ACM SIGKDD conference on knowledge discovery \& data mining},
  pages={1298--1308},
  year={2021}
}
@article{liu2021semi,
  title={Semi-supervised anomaly detection with dual prototypes autoencoder for industrial surface inspection},
  author={Liu, Jie and Song, Kechen and Feng, Mingzheng and Yan, Yunhui and Tu, Zhibiao and Zhu, Liu},
  journal={Optics and Lasers in Engineering},
  volume={136},
  pages={106324},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{de2021semi,
  title={A Semi-Supervised Bayesian Anomaly Detection Technique for Diagnosing Faults in Industrial IoT Systems},
  author={De Vita, Fabrizio and Bruneo, Dario and Das, Sajal K},
  booktitle={2021 IEEE International Conference on Smart Computing (SMARTCOMP)},
  pages={31--38},
  year={2021},
  organization={IEEE}
}

@article{chen2020unsupervised,
  title={Unsupervised anomaly detection of industrial robots using sliding-window convolutional variational autoencoder},
  author={Chen, Tingting and Liu, Xueping and Xia, Bizhong and Wang, Wei and Lai, Yongzhi},
  journal={IEEE Access},
  volume={8},
  pages={47072--47081},
  year={2020},
  publisher={IEEE}
}

@article{cui2022survey,
  title={A survey on unsupervised industrial anomaly detection algorithms},
  author={Cui, Yajie and Liu, Zhaoxiang and Lian, Shiguo},
  journal={arXiv preprint arXiv:2204.11161},
  year={2022}
}

@article{fraser2022challenges,
  title={Challenges for unsupervised anomaly detection in particle physics},
  author={Fraser, Katherine and Homiller, Samuel and Mishra, Rashmish K and Ostdiek, Bryan and Schwartz, Matthew D},
  journal={Journal of High Energy Physics},
  volume={2022},
  number={3},
  pages={1--31},
  year={2022},
  publisher={Springer}
}

article{ergen2019unsupervised,
  title={Unsupervised anomaly detection with LSTM neural networks},
  author={Ergen, Tolga and Kozat, Suleyman Serdar},
  journal={IEEE transactions on neural networks and learning systems},
  volume={31},
  number={8},
  pages={3127--3141},
  year={2019},
  publisher={IEEE}
}
@article{blazquez2021review,
  title={A review on outlier/anomaly detection in time series data},
  author={Bl{\'a}zquez-Garc{\'\i}a, Ane and Conde, Angel and Mori, Usue and Lozano, Jose A},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={3},
  pages={1--33},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{ergen2019unsupervised,
  title={Unsupervised anomaly detection with LSTM neural networks},
  author={Ergen, Tolga and Kozat, Suleyman Serdar},
  journal={IEEE transactions on neural networks and learning systems},
  volume={31},
  number={8},
  pages={3127--3141},
  year={2019},
  publisher={IEEE}
}

@article{yang2022learning,
  title={Learning deep feature correspondence for unsupervised anomaly detection and segmentation},
  author={Yang, Jie and Shi, Yong and Qi, Zhiquan},
  journal={Pattern Recognition},
  volume={132},
  pages={108874},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{usmani2022review,
  title={A Review of Unsupervised Machine Learning Frameworks for Anomaly Detection in Industrial Applications},
  author={Usmani, Usman Ahmad and Happonen, Ari and Watada, Junzo},
  booktitle={Intelligent Computing: Proceedings of the 2022 Computing Conference, Volume 2},
  pages={158--189},
  year={2022},
  organization={Springer}
}

@article{alimohammadi2022performance,
  title={Performance evaluation of outlier detection techniques in production timeseries: A systematic review and meta-analysis},
  author={Alimohammadi, Hamzeh and Chen, Shengnan Nancy},
  journal={Expert Systems with Applications},
  volume={191},
  pages={116371},
  year={2022},
  publisher={Elsevier}
}

@article{talagala2021anomaly,
  title={Anomaly detection in high-dimensional data},
  author={Talagala, Priyanga Dilini and Hyndman, Rob J and Smith-Miles, Kate},
  journal={Journal of Computational and Graphical Statistics},
  volume={30},
  number={2},
  pages={360--374},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{hilal2022financial,
  title={Financial Fraud:: A Review of Anomaly Detection Techniques and Recent Advances},
  author={Hilal, Waleed and Gadsden, S Andrew and Yawney, John},
  year={2022}
}

@article{agrawal2015survey,
  title={Survey on anomaly detection using data mining techniques},
  author={Agrawal, Shikha and Agrawal, Jitendra},
  journal={Procedia Computer Science},
  volume={60},
  pages={708--713},
  year={2015},
  publisher={Elsevier}
}

@article{yan2023hybrid,
  title={Hybrid robust convolutional autoencoder for unsupervised anomaly detection of machine tools under noises},
  author={Yan, Shen and Shao, Haidong and Xiao, Yiming and Liu, Bin and Wan, Jiafu},
  journal={Robotics and Computer-Integrated Manufacturing},
  volume={79},
  pages={102441},
  year={2023},
  publisher={Elsevier}
}
@article{zhang2023hybrid,
  title={A hybrid anomaly detection method for high dimensional data},
  author={Zhang, Xin and Wei, Pingping and Wang, Qingling},
  journal={PeerJ Computer Science},
  volume={9},
  pages={e1199},
  year={2023},
  publisher={PeerJ Inc.}
}

@article{mishne2019diffusion,
  title={Diffusion nets},
  author={Mishne, Gal and Shaham, Uri and Cloninger, Alexander and Cohen, Israel},
  journal={Applied and Computational Harmonic Analysis},
  volume={47},
  number={2},
  pages={259--285},
  year={2019},
  publisher={Elsevier}
}

@article{lu2019exploiting,
  title={Exploiting embedding manifold of autoencoders for hyperspectral anomaly detection},
  author={Lu, Xiaoqiang and Zhang, Wuxia and Huang, Ju},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={58},
  number={3},
  pages={1527--1537},
  year={2019},
  publisher={IEEE}
}

@phdthesis{moon2010design,
  title={Design and analysis of computer experiments for screening input variables},
  author={Moon, Hyejung},
  year={2010},
  school={The Ohio State University}
}

@article{morris1993bayesian,
  title={Bayesian design and analysis of computer experiments: use of derivatives in surface prediction},
  author={Morris, Max D and Mitchell, Toby J and Ylvisaker, Donald},
  journal={Technometrics},
  volume={35},
  number={3},
  pages={243--255},
  year={1993},
  publisher={Taylor \& Francis}
}

@inproceedings{breunig2000lof,
  title={LOF: identifying density-based local outliers},
  author={Breunig, Markus M and Kriegel, Hans-Peter and Ng, Raymond T and Sander, J{\"o}rg},
  booktitle={Proceedings of the 2000 ACM SIGMOD international conference on Management of data},
  pages={93--104},
  year={2000}
}

@article{eweis2022data,
  title={Data Fusion With Latent Map Gaussian Processes},
  author={Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={144},
  number={9},
  pages={091703},
  year={2022},
  publisher={American Society of Mechanical Engineers}
}

@article{egger2016hybrid,
  title={Hybrid organic--inorganic perovskites on the move},
  author={Egger, David A and Rappe, Andrew M and Kronik, Leeor},
  journal={Accounts of chemical research},
  volume={49},
  number={3},
  pages={573--581},
  year={2016},
  publisher={ACS Publications}
}

==> 17_Data_availability.tex <==
\section*{Code and Data Availability} \label{sec: availability}

 
